AdaCrowd: Unlabeled Scene Adaptation for Crowd Counting

We address the problem of image-based crowd counting. In particular, we propose a new problem called unlabeled scene-adaptive crowd counting. Given a new target scene, we would like to have a crowd counting model specifically adapted to this particular scene based on the target data that capture some information about the new scene. In this paper, we propose to use one or more unlabeled images from the target scene to perform the adaptation. In comparison with the existing problem setups (e.g. fully supervised), our proposed problem setup is closer to the real-world applications of crowd counting systems. We introduce a novel AdaCrowd framework to solve this problem. Our framework consists of a crowd counting network and a guiding network. The guiding network predicts some parameters in the crowd counting network based on the unlabeled images from a particular scene. This allows our model to adapt to different target scenes. The experimental results on several challenging benchmark datasets demonstrate the effectiveness of our proposed approach compared with other alternative methods. Code is available at https://github.com/maheshkkumar/adacrowd.

==> figures/bn_layers.tex <==
\begin{table}
	\label{fig:bn_layers}
	\centering
    \begin{tabular}{ccccc}
     	& (a) No BN & (b) BN &  (c) GBN \\
        & \includegraphics[width=0.11\linewidth]{images/without_bn.pdf} & \includegraphics[width=0.11\linewidth]{images/with_bn.pdf} & \includegraphics[width=0.285\linewidth]{images/with_gbn.pdf} \\
    \end{tabular}
	\caption{Without BN vs. With BN vs. With GBN}
\end{table}


==> figures/data.tex <==
\begin{table}
	\label{tab:metadata}
	\centering
    \begin{tabular}{ll|rrr}
        & \includegraphics[width=0.45 \linewidth]{images/rgb_metadata.pdf} & \includegraphics[width=0.45 \linewidth]{images/depth_metadata.pdf} & \\
    \end{tabular}
	\caption{Overview of different meta-data information we use in our approach. \textit{Left}: Unlabeled RGB images. \textit{Right}: Corresponding depth images for different datasets.}
\end{table}


==> figures/performance_vs_scenes.tex <==
\begin{figure}
	\centering
	{\setlength{\tabcolsep}{0.5pt}
		\begin{tabular}{cccc}
			\includegraphics[height=0.8in, width=1in]{plots/csrnet_mae.png}
			\includegraphics[height=0.8in, width=1in]{plots/csrnet_rmse.png}
			\\
		\end{tabular}
	}
	\caption{MAE/RMSE vs. Number of training scenes [[TODO]]}
	\label{fig:failure_cases}
\end{figure}


==> figures/placeholder.tex <==
\begin{table*}
	\label{tab:qualitative}
	\centering
    \begin{tabular}{ccccc}
     	& a & b & c & d \\
        1 & \includegraphics[width=0.2\linewidth]{images/placeholder.pdf} & \includegraphics[width=0.2\linewidth]{images/placeholder.pdf} & \includegraphics[width=0.2\linewidth]{images/placeholder.pdf} & \includegraphics[width=0.2\linewidth]{images/placeholder.pdf} \\
		 2 & \includegraphics[width=0.2\linewidth]{images/placeholder.pdf} & \includegraphics[width=0.2\linewidth]{images/placeholder.pdf} & \includegraphics[width=0.2\linewidth]{images/placeholder.pdf} & \includegraphics[width=0.2\linewidth]{images/placeholder.pdf} \\
		  3 & \includegraphics[width=0.2\linewidth]{images/placeholder.pdf} & \includegraphics[width=0.2\linewidth]{images/placeholder.pdf} & \includegraphics[width=0.2\linewidth]{images/placeholder.pdf} & \includegraphics[width=0.2\linewidth]{images/placeholder.pdf} \\
		   4 & \includegraphics[width=0.2\linewidth]{images/placeholder.pdf} & \includegraphics[width=0.2\linewidth]{images/placeholder.pdf} & \includegraphics[width=0.2\linewidth]{images/placeholder.pdf} & \includegraphics[width=0.2\linewidth]{images/placeholder.pdf} \\
    \end{tabular}
	\caption{Qualitative results}
\end{table*}


==> figures/problem_setup.tex <==
\begin{figure*}[!htb]
	\label{fig:problem_setup}
	\centering
	\begin{tabular}[t]{cc}
		\begin{tabular}{c}
			\smallskip
			\begin{subfigure}[t]{0.4\textwidth}
				\centering
				\includegraphics[width=\textwidth]{images/data_setup_v4.pdf}
				\caption{}
			\end{subfigure}\\
		\end{tabular}
		&
		\begin{tabular}{c}% if you add [t], than sub images are pushed down
			\smallskip
			\begin{subfigure}[t]{0.4\textwidth}
				\centering
				\includegraphics[width=0.9\textwidth]{images/supervised_v1.pdf}
				\caption{}
			\end{subfigure} \\
%			\hline
%			\\
			\begin{subfigure}[t]{0.4\textwidth}
				\centering
				\includegraphics[width=0.9\textwidth]{images/one_shot_v1.pdf}
				\caption{}
			\end{subfigure}
		\\  
%			\\ \hline
		\\
			\begin{subfigure}[t]{0.4\textwidth}
				\centering
				\includegraphics[width=0.9\textwidth]{images/unsupervised_v1.pdf}
				\caption{}
			\end{subfigure}
		\end{tabular}\\
	\end{tabular}
	\caption{Illustration of our AdaCrowd problem setting. (a) Overview of the training and test data set up for scene-based crowd counting. The test scene are completely different from the training scenes. (b) In a supervised learning approach, the model $f_{\theta}$ requires sufficient number of labled data to learn about the target scene. (c) In one-shot learning regime, the mode $f_{\theta}$ just requires one labeled data point to generate scene specific model parameters $\theta^{\ast}$ (d) In our AdaCrowd framework, we overcome thee requirement of labeled data and propose an effective approach to adapt a model $f_{
	\theta}$ to a target scene using meta-information (i.e., either a unlabeled image or depth map).}
\end{figure*}

==> figures/qualitative_bak.tex <==
\begin{figure*}
	\centering
    \begin{tabular}{ccccc}
     	& Ground truth & ResNet SFCN & ResNet SFCN w/ BN & \textbf{Ours (RGB)} \\
        WorldExpo S1 & \includegraphics[width=0.2\linewidth]{images/dataset/WE/GBN/25_gt.jpg} & \includegraphics[width=0.2\linewidth]{images/dataset/WE/Wo_BN/87.jpg} & \includegraphics[width=0.2\linewidth]{images/dataset/WE/BN/87.jpg} & \includegraphics[width=0.2\linewidth]{images/dataset/WE/GBN/25.jpg} \\
		 %WorldExpo S2  & \includegraphics[width=0.2\linewidth]{images/dataset/WE/GBN/148_gt.jpg} & \includegraphics[width=0.2\linewidth]{images/dataset/WE/Wo_BN/142.jpg} & \includegraphics[width=0.2\linewidth]{images/dataset/WE/BN/142.jpg} & \includegraphics[width=0.2\linewidth]{images/dataset/WE/GBN/148.jpg} \\
		  WorldExpo S3 & \includegraphics[width=0.2\linewidth]{images/dataset/WE/GBN/241_gt.jpg} & \includegraphics[width=0.2\linewidth]{images/dataset/WE/Wo_BN/264.jpg} & \includegraphics[width=0.2\linewidth]{images/dataset/WE/BN/264.jpg} & \includegraphics[width=0.2\linewidth]{images/dataset/WE/GBN/241.jpg} \\
		   %WorldExpo S4 & \includegraphics[width=0.2\linewidth]{images/dataset/WE/GBN/460_gt.jpg} & \includegraphics[width=0.2\linewidth]{images/dataset/WE/Wo_BN/361.jpg} & \includegraphics[width=0.2\linewidth]{images/dataset/WE/BN/361.jpg} & \includegraphics[width=0.2\linewidth]{images/dataset/WE/GBN/460.jpg} \\
		   %WorldExpo S5 & \includegraphics[width=0.2\linewidth]{images/dataset/WE/GBN/568_gt.jpg} & \includegraphics[width=0.2\linewidth]{images/dataset/WE/Wo_BN/576.jpg} & \includegraphics[width=0.2\linewidth]{images/dataset/WE/BN/576.jpg} & \includegraphics[width=0.2\linewidth]{images/dataset/WE/GBN/568.jpg} \\
		   Mall & \includegraphics[width=0.2\linewidth]{images/dataset/Mall/GBN/46_gt.jpg} & \includegraphics[width=0.2\linewidth]{images/dataset/Mall/Wo_BN/46.jpg} & \includegraphics[width=0.2\linewidth]{images/dataset/Mall/BN/46.jpg} & \includegraphics[width=0.2\linewidth]{images/dataset/Mall/GBN/46.jpg} \\
		   %PETS V1 & \includegraphics[width=0.2\linewidth]{images/dataset/PETS/GBN/189_gt.jpg} & \includegraphics[width=0.2\linewidth]{images/dataset/PETS/Wo_BN/476.jpg} & \includegraphics[width=0.2\linewidth]{images/dataset/PETS/BN/476.jpg} & \includegraphics[width=0.2\linewidth]{images/dataset/PETS/GBN/189.jpg} \\
		    %FDST S1& \includegraphics[width=0.2\linewidth]{images/dataset/FDST/GBN/245_gt.jpg} & \includegraphics[width=0.2\linewidth]{images/dataset/FDST/wo_BN/287.jpg} & \includegraphics[width=0.2\linewidth]{images/dataset/FDST/BN/287.jpg} & \includegraphics[width=0.2\linewidth]{images/dataset/FDST/GBN/245.jpg} \\
    \end{tabular}
	\caption{Qualitative results}
	\label{fig:qualitative}
\end{figure*}


==> learning.tex <==
\subsection{Learning and Inference}\label{sec:learning}
Note that the counting network is parameterized by $\{\phi, \psi\}$. But the model parameters we need to learn are $\{\psi, \theta\}$, since $\phi$ will be directly predicted from the guiding network (see Eq.~\ref{eq:gbn}). We would like to learn model parameters that have the following property. Suppose we have a new scene represented by $z$ (unlabeled image). We would like the counting network with GBN parameters $\phi$ obtained via Eq.~\ref{eq:gbn} to perform well on images from this scene. To achieve this, we learn the model parameters from a set of labeled training images collected from multiple scenes. The model parameters are learned in a way that is amenable to effective adaptation to a new scene based on its scene-specific unlabeled data $z$.

The learning algorithm works iteratively. In each iteration, the algorithm constructs a unlabeled scene adaptation task that mimics the scenario during testing. For a scene $\mathcal{S}^{t}$, we use $\{(x_1,y_1),...,(x_N,y_N)\}$ to denote the $N$ training examples from this scene, where $(x_i,y_i)$ correspond to the $i$-th (image, label) pair. We construct the task as follows. We randomly select one image to construct the scene-specific unlabeled data $z$. %In the case of $z$ being the depth map, we simply use an off-the-shelf depth estimation algorithm~\cite{li2018megadepth} to get the depth map. 
Without loss of generality, let us assume that $x_1$ is selected to construct $z$. We feed $z$ to Eq.~\ref{eq:gbn} to compute the GBN parameters $\phi$ from the guiding network parameterized by $\theta$. We then define a loss function that measures the ``goodness'' of the counting network with parameters $\{\phi, \psi\}$. Since our goal is for the learned model to perform well on other images from the same scene, a reasonable loss function is to measure the performance on the remaining $N-1$ images from this scene. We can define the loss for this scene $\mathcal{S}^{t}$ as follows:
\begin{subeqnarray}
  \label{eq:loss_scene}
  \hspace{-30pt}\mathcal{L}(\{\psi,\theta\}; \mathcal{S}^t)&&\hspace{5pt}=\sum_{i=2}^{N}||f(x_i; \{\phi,\psi\})-y_i||^2\\
  \hspace{-30pt} &&\hspace{5pt}=\sum_{i=2}^{N}||f(x_i; \{g(z;\theta), \psi\})-y_i||^2
\end{subeqnarray}
Here we use the $L_2$ distance to measure the difference between the predicted (i.e. $f(x_i; \{g(z;\theta), \psi\})$) and the ground-truth (i.e. $y_i$) density maps. 

The overall objective is to learn $\{\psi,\theta\}$ that minimize Eq.~\ref{eq:loss_scene} across all scenes during training, i.e.:
\begin{eqnarray}
  \label{eq:loss_all}
  &&\min_{\{\psi,\theta\}}\sum_{t}\mathcal{L}(\{\psi,\theta\}; \mathcal{S}^t)
\end{eqnarray}
In Eq.~\ref{eq:loss_all}, we sum over the loss across all scenes to optimize the parameters during training. %In practice, we sample a mini-batch of images from every scene to optimize the parameters.
In Algorithm~\ref{algo:unsupervised_adaptation}, we provide an overview of the learning mechanism.

\input{algorithm}

Let $\{\psi^*, \theta^*\}$ be the learned model parameters that minimize Eq.~\ref{eq:loss_all}. During testing, we are given a new scene represented as $z_{new}$ (unlabeled image). For any crowd image $x$ from this scene, we can predict its label $\hat{y}$ as:
\begin{equation}
  \hat{y}=f(x; \{\phi^*, \psi^*\}), \textrm{ where } \phi^*=g(z_{new};\theta^*)
\end{equation}

%\input{figures/bn_layers}


==> results.tex <==
% Results

==> tables/shot_1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
	\centering
	\small
	\begin{tabular}{|l|l|c|c|c|c|c|}
		\hline
		\multicolumn{7}{|c|}{K=1}                                                                     \\ \hline
		Source $\rightarrow$ Target          & Model                  & MAE $(\downarrow)$ & MSE $(\downarrow)$ & MDE $(\downarrow)$ & PSNR $(\uparrow)$ & SSIM $(\uparrow)$\\ \hline
		
		% CSRNet: WE
		\multirow{9}{*}{WE $\rightarrow$ WE} & CSRNet                 &19.56     &28.34     & 0.415    & 28.5     &      \\ 
		& CSRNet w/ BN            & 18.57    & 29.91    &  0.28   &   30.88   &      \\ 
		& {\fontfamily{qcr}\selectfont AdaCrowd} + RGB (Ours)        & \textbf{17.32 $\pm {\tiny 0.1} \% $}     & \textbf{27.03 $\pm {\tiny 0.05} \% $}     &  \textbf{0.526 $\pm {\tiny 1.15} \% $}   &   \textbf{30.15 $\pm {\tiny 0.1} \% $}   &      \\ 
		& {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours)        & \textbf{17.66 $\pm {\tiny 0.8} \% $}     & \textbf{27.18 $\pm {\tiny 0.4} \% $}     &  \textbf{0.432 $\pm {\tiny 0.3} \% $}   &   \textbf{30.31 $\pm {\tiny 0.2} \% $}   &      \\ \cline{2-7}
		
		% ResNet: WE
		& ResNet101              & 23.07    & 34.16    &  0.357   &  28.09    &      \\ 
		& ResNet101 w/ BN         & 21.65    & 33.3    &  0.33   &      &      \\ 
		& {\fontfamily{qcr}\selectfont AdaCrowd} + RGB (Ours)      & \textbf{20.91 $\pm {\tiny 0.3} \% $}    & \textbf{29.61 $\pm {\tiny 0.2} \% $}    & \textbf{1.18 $\pm {\tiny 2.0} \% $}    &   \textbf{27.84 $\pm {\tiny 0.06} \% $}   &      \\ 
		& {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours)        & \textbf{20.28 $\pm {\tiny 0.4} \% $}     & \textbf{29.83 $\pm {\tiny 0.1} \% $}     &  \textbf{0.9 $\pm {\tiny 0.1} \% $}   &   \textbf{28.56 $\pm {\tiny 0.3} \% $}   &      \\ \cline{2-7} 
		
		% ResNet SFCN: WE
		& ResNet101 SFCN         &   25.47  & 35.91    &  0.378   &      &      \\ 
		& ResNet101 SFCN w/ BN & 23.84   & 35.52    & 0.374    &     &      \\ 
		& {\fontfamily{qcr}\selectfont AdaCrowd} + RGB (Ours) & \textbf{14.56 $\pm {\tiny 0.4} \% $}    & \textbf{22.75 $\pm {\tiny 0.2} \% $}    &  \textbf{0.352 $\pm {\tiny 3.0} \% $}   &  \textbf{32.2 $\pm {\tiny 0.1} \% $}    &      \\ 
		& {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours)        & \textbf{13.66 $\pm {\tiny 1.0} \% $}     & \textbf{22.92 $\pm {\tiny 1.6} \% $}     &  \textbf{0.271 $\pm {\tiny 0.3} \% $}   &   \textbf{32.89 $\pm {\tiny 0.1} \% $}   &      \\ \hline
		
		% CSRNet: Mall
		\multirow{9}{*}{WE $\rightarrow$ Mall} & CSRNet                 & 9.94    & 10.41    &  0.329   &  28.77    &      \\ 
		& CSRNet w/ BN            & 8.72    & 9.92    &  0.267   &  29.9    &      \\ 
		& {\fontfamily{qcr}\selectfont AdaCrowd} + RGB (Ours)        & \textbf{4.0 $\pm {\tiny 0.08} \% $}    & \textbf{5.0 $\pm {\tiny 0.09} \% $}    &  \textbf{0.130 $\pm {\tiny 0.08} \% $}   &  \textbf{39.6 $\pm {\tiny 0.07} \% $}    &      \\ 
		& {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours)        & \textbf{3.5 $\pm {\tiny 0.1} \% $}     & \textbf{4.4 $\pm {\tiny 0.09} \% $}     &  \textbf{0.111 $\pm {\tiny 0.3} \% $}   &   \textbf{40.8 $\pm {\tiny 0.1} \% $}   &      \\ \cline{2-7}
		
		% ResNet: Mall 
		& ResNet101              & 9.03    & 9.6    &  0.279   &  29.68   &      \\ 
		& ResNet101 w/ BN         & 9.63    & 10.32    &  0.296   &  29.50    &      \\ 
		& {\fontfamily{qcr}\selectfont AdaCrowd} + RGB (Ours)      &  \textbf{4.12 $\pm {\tiny 0.2} \% $}   & \textbf{5.12 $\pm {\tiny 0.2} \% $}    &  \textbf{0.134 $\pm {\tiny 0.3} \% $}   &  \textbf{39.24 $\pm {\tiny 0.08} \% $}    &      \\ & {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours)        & \textbf{6.5 $\pm {\tiny 1.2} \% $}     & \textbf{7.5 $\pm {\tiny 1.0} \% $}     &  \textbf{0.218 $\pm {\tiny 1.2} \% $}   &   \textbf{39.24 $\pm {\tiny 0.08} \% $}   &      \\ \cline{2-7}
		
		% ResNet SFCN: Mall 
		& ResNet101 SFCN         &  15.17   &  15.53   &  0.471   &      &      \\ 
		& ResNet101 SFCN w/ BN    & 10.8    &  11.39   &  0.335   &      &      \\ 
		& {\fontfamily{qcr}\selectfont AdaCrowd} + RGB (Ours) &  \textbf{6.99 $\pm {\tiny 1.2} \% $}   & \textbf{8.0 $\pm {\tiny 1.0} \% $}    &  \textbf{0.237 $\pm {\tiny 1.2} \% $}   &  \textbf{33.6 $\pm {\tiny 0.03} \% $}   & \\ 
		& {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours)        & \textbf{8.32$\pm {\tiny 0.1} \% $}     & \textbf{9.24 $\pm {\tiny 0.1} \% $}     &  \textbf{0.277 $\pm {\tiny 0.2} \% $}   &   \textbf{31.24 $\pm {\tiny 0.07} \% $}   &      \\ \hline
		
		% CSRNet: PETS
		\multirow{9}{*}{WE $\rightarrow$ PETS} & CSRNet                 &  17.99   &  19.8  &  0.646  &  25.07   &      \\ 
		& CSRNet w/ BN            &  18.63   &  20.49   &  0.670   &  24.74    &      \\ 
		& {\fontfamily{qcr}\selectfont AdaCrowd} + RGB (Ours)        &  \textbf{18.77 $\pm {\tiny 0.0} \%$}   &  \textbf{20.09 $\pm {\tiny 0.0} $}   &     &      &      \\ 
		& {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours)        & \textbf{- $\pm {\tiny 0.0} \% $}     & \textbf{- $\pm {\tiny 0.0} \% $}     &  \textbf{- $\pm {\tiny 0.0} \% $}   &   \textbf{- $\pm {\tiny 0.0} \% $}   &      \\\cline{2-7} 
		
		% ResNet: PETS
		& ResNet101              &  20.38   & 22.67    & 0.722   &  24.59   &      \\ 
		& ResNet101 w/ BN         &  19.59   &  21.61   &  0.718  &  24.28   &      \\ 
		& {\fontfamily{qcr}\selectfont AdaCrowd} + RGB (Ours)        & \textbf{13.74 $\pm {\tiny 0.1} \% $}     & \textbf{16.15 $\pm {\tiny 0.09} \% $}     &  \textbf{0.482 $\pm {\tiny 0.139} \% $}   &   \textbf{28.43 $\pm {\tiny 0.07} \% $}   &     \\ 
		& {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours)        & \textbf{19.56 $\pm {\tiny 3.1} \% $}     & \textbf{21.52 $\pm {\tiny 2.5} \% $}     &  \textbf{0.718 $\pm {\tiny 3.7} \% $}   &   \textbf{- $\pm {\tiny 0.0} \% $}   &      \\ \cline{2-7} 
		
		% ResNet SFCN: PETS
		& ResNet101 SFCN         &  19.62   &  21.55   &  0.708   &      &      \\ 
		& ResNet101 SFCN w/ BN    &  19.94   &  22.26   &  0.718   &  24.48  &      \\ 
		& {\fontfamily{qcr}\selectfont AdaCrowd} + RGB (Ours) & \textbf{18.41 $\pm {\tiny 0.2} $}  & \textbf{20.63 $\pm {\tiny 0.1} $}    &  \textbf{0.653 $\pm {\tiny 0.2} $}   &   \textbf{25.32 $\pm {\tiny 0.1} $}   & \\ 
		& {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours)        & \textbf{13.74 $\pm {\tiny 0.1} \% $}     & \textbf{16.15 $\pm {\tiny 0.09} \% $}     &  \textbf{0.482 $\pm {\tiny 0.139} \% $}   &   \textbf{28.43 $\pm {\tiny 0.07} \% $}   &      \\ \hline
		
		% CSRNet: FDST
		\multirow{9}{*}{WE $\rightarrow$ FUDAN} & CSRNet      &       12.74    &  13.09   &  0.607   &  30.80   &  \\ 
		& CSRNet w/ BN            &   6.44 &  6.81   & 0.272    &  34.73    &      \\ 
		& {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours)        &  \textbf{- $\pm {\tiny 0.0} $}   &   \textbf{- $\pm {\tiny 0.0} $}  &  \textbf{- $\pm {\tiny 0.0} $}   &  \textbf{- $\pm {\tiny 0.0} $}    &      \\ 
		& {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours)        & \textbf{- $\pm {\tiny 0.0} \% $}     & \textbf{- $\pm {\tiny 0.0} \% $}     &  \textbf{- $\pm {\tiny 0.0} \% $}   &   \textbf{- $\pm {\tiny 0.0} \% $}   &      \\ \cline{2-7} 
		
		% ResNet: FDST
		& ResNet101              &  6.81   &  7.19  &  0.26  &  35.02    &      \\ 
		& ResNet101 w/ BN         &  8.89   &  9.23   &  0.332  &  32.11   &      \\ 
		& {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours)      &  \textbf{6.13 $\pm {\tiny 0.4} $}   & \textbf{6.69 $\pm {\tiny 0.3} $}    & \textbf{0.406 $\pm {\tiny 0.4} $}    &  \textbf{- $\pm {\tiny 0.0} $}    &      \\ 
		& {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours)        & \textbf{- $\pm {\tiny 0.0} \% $}     & \textbf{- $\pm {\tiny 0.0} \% $}     &  \textbf{- $\pm {\tiny 0.0} \% $}   &   \textbf{- $\pm {\tiny 0.0} \% $}   &      \\ \cline{2-7} 
		
		% ResNet SFCN: FDST
		& ResNet101 SFCN         &  4.51   &  4.85   &  0.186   &   39.7   &      \\ 
		& ResNet101 SFCN w/ BN    &  4.8   &  5.21   &  0.207   &  38.47   &      \\ 
		& {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours) &  \textbf{- $\pm {\tiny 0.0} $}   &  \textbf{- $\pm {\tiny 0.0} $}   &  \textbf{- $\pm {\tiny 0.0} $}   &  \textbf{- $\pm {\tiny 0.0} $}    & \\ 
		& {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours)        & \textbf{- $\pm {\tiny 0.0} \% $}     & \textbf{- $\pm {\tiny 0.0} \% $}     &  \textbf{- $\pm {\tiny 0.0} \% $}   &   \textbf{- $\pm {\tiny 0.0} \% $}   &      \\ \hline
	\end{tabular}
	\label{tab:quantitative_k1}
	\caption{Results for AdaCrowd for K=1 from WorldExpo to Mall, UCSD, PETS and FDST [[TODO]]}
\end{table*}

==> tables/shot_5.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
	\centering
	\small
	\begin{tabular}{|l|l|l|l|l|l|l|}
		\hline
		\multicolumn{7}{|c|}{K=5}                                                                     \\ \hline
		Source $\rightarrow$ Target          & Model                  & MAE $(\downarrow)$ & MSE $(\downarrow)$ & MDE $(\downarrow)$ & PSNR $(\uparrow)$ & SSIM $(\uparrow)$\\ \hline
		\multirow{9}{*}{WE $\rightarrow$ WE} & CSRNet                 &     &     &     &      &      \\ 
		& CSRNet w/ BN            &     &     &     &      &      \\ 
		& CSRNet w/ AdaBN (Ours)        &     &     &     &      &      \\ \cline{2-7} 
		& ResNet101              &     &     &     &      &      \\ 
		& ResNet101 w/ BN         &     &     &     &      &      \\ 
		& ResNet101 w/ AdaBN (Ours)      &     &     &     &      &      \\ \cline{2-7} 
		& ResNet101 SFCN         &     &     &     &      &      \\ 
		& ResNet101 SFCN w/ BN    &     &     &     &      &      \\ 
		& ResNet101 SFCN w/ AdaBN (Ours) &     &     &     &      &      \\ \hline
		\multirow{9}{*}{WE $\rightarrow$ Mall} & CSRNet                 &     &     &     &      &      \\ 
		& CSRNet w/ BN            &     &     &     &      &      \\ 
		& CSRNet w/ AdaBN (Ours)        &     &     &     &      &      \\ \cline{2-7} 
		& ResNet101              &     &     &     &      &      \\ 
		& ResNet101 w/ BN         &     &     &     &      &      \\ 
		& ResNet101 w/ AdaBN (Ours)      &     &     &     &      &      \\ \cline{2-7} 
		& ResNet101 SFCN         &     &     &     &      &      \\ 
		& ResNet101 SFCN w/ BN    &     &     &     &      &      \\ 
		& ResNet101 SFCN w/ AdaBN (Ours) &     &     &     &      & \\      
		& Fully supervised (Oracle) &     &     &     &      &  \\ \hline
		\multirow{9}{*}{WE $\rightarrow$ PETS} & CSRNet                 &     &     &     &      &      \\ 
		& CSRNet w/ BN            &     &     &     &      &      \\ 
		& CSRNet w/ AdaBN (Ours)        &     &     &     &      &      \\ \cline{2-7} 
		& ResNet101              &     &     &     &      &      \\ 
		& ResNet101 w/ BN         &     &     &     &      &      \\ 
		& ResNet101 w/ AdaBN (Ours)      &     &     &     &      &      \\ \cline{2-7} 
		& ResNet101 SFCN         &     &     &     &      &      \\ 
		& ResNet101 SFCN w/ BN    &     &     &     &      &      \\ 
		& ResNet101 SFCN w/ AdaBN (Ours) &     &     &     &      & \\      
		& Fully supervised (Oracle) &     &     &     &      &  \\ \hline
		\multirow{9}{*}{WE $\rightarrow$ FDST} & CSRNet                 &     &     &     &      &      \\ 
		& CSRNet w/ BN            &     &     &     &      &      \\ 
		& CSRNet w/ AdaBN (Ours)        &     &     &     &      &      \\ \cline{2-7} 
		& ResNet101              &     &     &     &      &      \\ 
		& ResNet101 w/ BN         &     &     &     &      &      \\ 
		& ResNet101 w/ AdaBN (Ours)      &     &     &     &      &      \\ \cline{2-7} 
		& ResNet101 SFCN         &     &     &     &      &      \\ 
		& ResNet101 SFCN w/ BN    &     &     &     &      &      \\ 
		& ResNet101 SFCN w/ AdaBN (Ours) &     &     &     &      & \\      
		& Fully supervised (Oracle) &     &     &     &      &  \\ \hline
	\end{tabular}
	\label{tab:quantitative_k5}
\end{table*}

==> tables/tab_affine.tex <==
\begin{table*}[]
	\small
	\centering
	\caption{An analysis on the effect of affine parameters to scene adaptation}
	\begin{tabular}{||l|c|c||c|c||c|c||}
		\hline
		\multirow{2}{*}{\textbf{Models}} &
		 \multicolumn{2}{c||}{\textbf{WorldExpo} $\rightarrow$ \textbf{Mall}} & \multicolumn{2}{c||}{\textbf{WorldExpo} $\rightarrow$ \textbf{PETS}} & \multicolumn{2}{c||}{\textbf{WorldExpo} $\rightarrow$ \textbf{FDST}} \\ \cline{2-7} 
		& \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE}
		\\ \hline
		% ResNet: WE
		CSRNet w/ fixed $\gamma=1, \beta=0$   & 10.62  & 12.60 & 18.82  & 20.80 & 7.89  &  8.28 \\ 
		CSRNet w/ learable $\gamma, \beta$  &  8.72   &  9.92  & 18.63   & 20.49 &  7.30  & 7.81 \\ 
		\textbf{Ours (RGB) w/ CSRNet}      & \textbf{ 4.0 $\pm {\tiny 0.08}$}    & \textbf{5.0 $\pm {\tiny 0.09}$}  & \textbf{17.43 $\pm {\tiny 0.04}$}  & \textbf{19.70 $\pm {\tiny 0.05}$}  & \textbf{7.14 $\pm {\tiny 0.3}$}  & \textbf{7.70 $\pm {\tiny 0.2}$}   \\ \hline
	\end{tabular}
	\label{tab:affine}
\end{table*}


==> tables/tab_ours_vs_oracle.tex <==
\begin{table}[ht]
	\centering
	\caption{{\color{blue} Comparison with few-shot (oracle) adaptation networks on the WorldExpo'10 dataset that are based on the CSRNet~\cite{li2018csrnet} architecture.}}
	\tiny
	\renewcommand{\arraystretch}{1.1}
	\begin{tabular}{l|ccc}
%		\toprule
		\hline
		Method & Adaptation & MAE ($\downarrow$)   & RMSE ($\downarrow$) \\ \hline
		CSRNet ~\cite{li2018csrnet}             & No & 19.56     &28.34  \\ 
		CSRNet w/ BN~\cite{li2018csrnet}     &  No & 18.57    & 29.91 \\ 
%		CSRNet w/ BN~\cite{li2018csrnet} + FA & Unlabeled & 18.08 & 27.88\\ 
%		CSRNet w/ BN~\cite{li2018csrnet} + CS & Unlabeled & 19.13  & 27.57 \\  
		\textbf{Ours w/ CSRNet} + GBN & Unlabeled & \textbf{17.32}~\smaller{$\pm{0.1}$}     & \textbf{27.03} \smaller{$\pm {0.05}$}  \\ 
		\hline
		CSRNet w/ 1-shot~\cite{hossain2019one} & Labeled & {\color{gray} 8.23 } & {\color{gray} 12.08 }\\
		CSRNet w/ 1-shot~\cite{Reddy_2020_WACV} & Labeled & {\color{gray} 7.5 } & { \color{gray} 10.22 } \\
%         \bottomrule
		\hline
	\end{tabular}
    \label{tab:we_vs_oracle}
\end{table}


==> tables/tab_we_mall.tex <==
\begin{table*}[]
	\centering
	\caption{Quantitative results for WorldExpo to WorldExpo and WorldExpo to Mall}
%	\bgroup
%	\def\arraystretch{1.15}% 
	\begin{tabular}{||l|c|c||c|c||}
		\hline
		\multirow{2}{*}{\textbf{Models}} & \multicolumn{2}{c||}{\textbf{WorldExpo} $\rightarrow$ \textbf{WorldExpo}} & \multicolumn{2}{c||}{\textbf{WorldExpo} $\rightarrow$ to \textbf{Mall}} \\ \cline{2-5} 
		&  \textbf{MAE} $(\downarrow)$                   & \textbf{MSE} $(\downarrow)$                  & \textbf{MAE} $(\downarrow)$               & \textbf{MSE} $(\downarrow)$               \\ \hline
		 CSRNet ~\cite{li2018csrnet}                 &19.56     &28.34  & 9.94    & 10.41 \\ 
		 CSRNet w/ BN~\cite{li2018csrnet}            & 18.57    & 29.91 & 8.72    & 9.92 \\ 
		 {\fontfamily{qcr}\selectfont AdaCrowd} + RGB (\textbf{Ours})        & \textbf{\color{red}{17.32 $\pm {\tiny 0.1} \% $}}     & \textbf{\color{red}{27.03 $\pm {\tiny 0.05} \% $}} & \textbf{\color{blue}{4.0 $\pm {\tiny 0.08} \% $}}    & \textbf{\color{blue}{5.0 $\pm {\tiny 0.09} \% $}}     \\ 
		 {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (\textbf{Ours})        & \textbf{\color{blue}{17.66 $\pm {\tiny 0.8} \% $}}     & \textbf{\color{blue}{27.18 $\pm {\tiny 0.4} \% $}}    & \textbf{\color{red}{3.5 $\pm {\tiny 0.1} \% $}}     & \textbf{\color{red}{4.4 $\pm {\tiny 0.09} \% $}}      \\ \hline
		 
		 % ResNet: WE
		 ResNet101~\cite{he2016deep}              & 23.07    & 34.16 & 9.03    & 9.6    \\ 
		 ResNet101 w/ BN~\cite{he2016deep}         & 21.65    & 33.3    & 9.63    & 10.32    \\ 
		 {\fontfamily{qcr}\selectfont AdaCrowd} + RGB (\textbf{Ours})      & \textbf{\color{blue}{20.91 $\pm {\tiny 0.3} \% $}}    & \textbf{\color{red}{29.61 $\pm {\tiny 0.2} \% $}} &  \textbf{\color{red}{4.12 $\pm {\tiny 0.2} \% $}}   & \textbf{\color{red}{5.12 $\pm {\tiny 0.2} \% $}}   \\ 
		 {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (\textbf{Ours})        & \textbf{\color{red}{20.28 $\pm {\tiny 0.4} \% $}}     & \textbf{\color{blue}{29.83 $\pm {\tiny 0.1} \% $}}   & \textbf{\color{blue}{6.5 $\pm {\tiny 1.2} \% $}}     & \textbf{\color{blue}{7.5 $\pm {\tiny 1.0} \% $}}        \\ \hline
		 
		 % ResNet SFCN: WE
		 ResNet101 SFCN~\cite{wang2019learning}         &   25.47  & 35.91   &  15.17   &  15.53    \\ 
		 ResNet101 SFCN w/ BN~\cite{wang2019learning}  & 23.84   & 35.52  & 10.8    &  11.39    \\  
		 {\fontfamily{qcr}\selectfont AdaCrowd} + RGB (\textbf{Ours}) & \textbf{\color{blue}{14.56 $\pm {\tiny 0.4} \% $}}    & \textbf{\color{red}{22.75 $\pm {\tiny 0.2} \% $}} &  \textbf{\color{red}{6.99 $\pm {\tiny 1.2} \% $}}   & \textbf{\color{red}{8.0 $\pm {\tiny 1.0} \% $}}   \\ 
		 {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (\textbf{Ours})        & \textbf{\color{red}{13.66 $\pm {\tiny 1.0} \% $}}     & \textbf{\color{blue}{22.92 $\pm {\tiny 1.6} \% $}}  & \textbf{\color{blue}{8.32$\pm {\tiny 0.1} \% $}}     & \textbf{\color{blue}{9.24 $\pm {\tiny 0.1} \% $}}   \\ \hline
	\end{tabular}
\end{table*}

%\begin{table*}[]
%	\centering
%	\small
%	\begin{tabular}{|l|l|c|c|}
%		\hline
%		\multicolumn{4}{|c|}{K=1}                                                                     \\ \hline
%		Source $\rightarrow$ Target          & Model                  & MAE $(\downarrow)$ & MSE $(\downarrow)$ \\ \hline
%		
%		% CSRNet: WE
%		\multirow{12}{*}{WE $\rightarrow$ WE} & CSRNet                 &19.56     &28.34 \\ 
%		& CSRNet w/ BN            & 18.57    & 29.91 \\ 
%		& {\fontfamily{qcr}\selectfont AdaCrowd} + RGB (Ours)        & \textbf{17.32 $\pm {\tiny 0.1} \% $}     & \textbf{27.03 $\pm {\tiny 0.05} \% $} \\ 
%		& {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours)        & \textbf{17.66 $\pm {\tiny 0.8} \% $}     & \textbf{27.18 $\pm {\tiny 0.4} \% $}    \\ \cline{2-4}
%		
%		% ResNet: WE
%		& ResNet101              & 23.07    & 34.16 \\ 
%		& ResNet101 w/ BN         & 21.65    & 33.3    \\ 
%		& {\fontfamily{qcr}\selectfont AdaCrowd} + RGB (Ours)      & \textbf{20.91 $\pm {\tiny 0.3} \% $}    & \textbf{29.61 $\pm {\tiny 0.2} \% $} \\ 
%		& {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours)        & \textbf{20.28 $\pm {\tiny 0.4} \% $}     & \textbf{29.83 $\pm {\tiny 0.1} \% $}   \\ \cline{2-4} 
%		
%		% ResNet SFCN: WE
%		& ResNet101 SFCN         &   25.47  & 35.91   \\ 
%		& ResNet101 SFCN w/ BN & 23.84   & 35.52  \\ 
%		& {\fontfamily{qcr}\selectfont AdaCrowd} + RGB (Ours) & \textbf{14.56 $\pm {\tiny 0.4} \% $}    & \textbf{22.75 $\pm {\tiny 0.2} \% $}  \\ 
%		& {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours)        & \textbf{13.66 $\pm {\tiny 1.0} \% $}     & \textbf{22.92 $\pm {\tiny 1.6} \% $}    \\ \hline
%		
%		% CSRNet: Mall
%		\multirow{9}{*}{WE $\rightarrow$ Mall} & CSRNet                 & 9.94    & 10.41   \\ 
%		& CSRNet w/ BN            & 8.72    & 9.92   \\ 
%		& {\fontfamily{qcr}\selectfont AdaCrowd} + RGB (Ours)        & \textbf{4.0 $\pm {\tiny 0.08} \% $}    & \textbf{5.0 $\pm {\tiny 0.09} \% $}     \\ 
%		& {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours)        & \textbf{3.5 $\pm {\tiny 0.1} \% $}     & \textbf{4.4 $\pm {\tiny 0.09} \% $}      \\ \cline{2-4}
%		
%		% ResNet: Mall 
%		& ResNet101              & 9.03    & 9.6    \\ 
%		& ResNet101 w/ BN         & 9.63    & 10.32    \\ 
%		& {\fontfamily{qcr}\selectfont AdaCrowd} + RGB (Ours)      &  \textbf{4.12 $\pm {\tiny 0.2} \% $}   & \textbf{5.12 $\pm {\tiny 0.2} \% $}   \\ 
%		& {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours)        & \textbf{6.5 $\pm {\tiny 1.2} \% $}     & \textbf{7.5 $\pm {\tiny 1.0} \% $}        \\ \cline{2-4}
%		
%		% ResNet SFCN: Mall 
%		& ResNet101 SFCN         &  15.17   &  15.53    \\ 
%		& ResNet101 SFCN w/ BN    & 10.8    &  11.39    \\ 
%		& {\fontfamily{qcr}\selectfont AdaCrowd} + RGB (Ours) &  \textbf{6.99 $\pm {\tiny 1.2} \% $}   & \textbf{8.0 $\pm {\tiny 1.0} \% $}   \\ 
%		& {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours)        & \textbf{8.32$\pm {\tiny 0.1} \% $}     & \textbf{9.24 $\pm {\tiny 0.1} \% $}    \\ \hline
%		
%		% CSRNet: PETS
%		\multirow{9}{*}{WE $\rightarrow$ PETS} & CSRNet                 &  17.99   &  19.8   \\ 
%		& CSRNet w/ BN            &  18.63   &  20.49  \\ 
%		& {\fontfamily{qcr}\selectfont AdaCrowd} + RGB (Ours)        &  \textbf{18.77 $\pm {\tiny 0.0} \%$}   &  \textbf{20.09 $\pm {\tiny 0.0} $}  \\ 
%		& {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours)        & \textbf{- $\pm {\tiny 0.0} \% $}     & \textbf{- $\pm {\tiny 0.0} \% $}     \\\cline{2-4} 
%		
%		% ResNet: PETS
%		& ResNet101              &  20.38   & 22.67 \\ 
%		& ResNet101 w/ BN         &  19.59   &  21.61     \\ 
%		& {\fontfamily{qcr}\selectfont AdaCrowd} + RGB (Ours)        & \textbf{13.74 $\pm {\tiny 0.1} \% $}     & \textbf{16.15 $\pm {\tiny 0.09} \% $} \\ 
%		& {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours)        & \textbf{19.56 $\pm {\tiny 3.1} \% $}     & \textbf{21.52 $\pm {\tiny 2.5} \% $}   \\ \cline{2-4} 
%		
%		% ResNet SFCN: PETS
%		& ResNet101 SFCN         &  19.62   &  21.55  \\ 
%		& ResNet101 SFCN w/ BN    &  19.94   &  22.26  \\ 
%		& {\fontfamily{qcr}\selectfont AdaCrowd} + RGB (Ours) & \textbf{18.41 $\pm {\tiny 0.2} $}  & \textbf{20.63 $\pm {\tiny 0.1} $}   \\ 
%		& {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours)        & \textbf{13.74 $\pm {\tiny 0.1} \% $}     & \textbf{16.15 $\pm {\tiny 0.09} \% $}      \\ \hline
%		
%		% CSRNet: FDST
%		\multirow{9}{*}{WE $\rightarrow$ FUDAN} & CSRNet      &       12.74    &  13.09   \\ 
%		& CSRNet w/ BN            &   6.44 &  6.81   \\ 
%		& {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours)        &  \textbf{- $\pm {\tiny 0.0} $}   &   \textbf{- $\pm {\tiny 0.0} $}    \\ 
%		& {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours)        & \textbf{- $\pm {\tiny 0.0} \% $}     & \textbf{- $\pm {\tiny 0.0} \% $}       \\ \cline{2-4} 
%		
%		% ResNet: FDST
%		& ResNet101              &  6.81   &  7.19     \\ 
%		& ResNet101 w/ BN         &  8.89   &  9.23    \\ 
%		& {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours)      &  \textbf{6.13 $\pm {\tiny 0.4} $}   & \textbf{6.69 $\pm {\tiny 0.3} $}       \\ 
%		& {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours)        & \textbf{- $\pm {\tiny 0.0} \% $}     & \textbf{- $\pm {\tiny 0.0} \% $}    \\ \cline{2-4} 
%		
%		% ResNet SFCN: FDST
%		& ResNet101 SFCN         &  4.51   &  4.85   \\ 
%		& ResNet101 SFCN w/ BN    &  4.8   &  5.21   \\ 
%		& {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours) &  \textbf{- $\pm {\tiny 0.0} $}   &  \textbf{- $\pm {\tiny 0.0} $}  \\ 
%		& {\fontfamily{qcr}\selectfont AdaCrowd} + Depth (Ours)        & \textbf{- $\pm {\tiny 0.0} \% $}     & \textbf{- $\pm {\tiny 0.0} \% $}     \\ \hline
%	\end{tabular}
%	\label{tab:quantitative_k1}
%	\caption{Results for AdaCrowd for K=1 from WorldExpo to Mall, UCSD, PETS and FDST [[TODO]]}
%\end{table*}


==> tables/tab_we_other_5shot.tex <==
\begin{table*}[]
	\centering
	\caption{Quantitative results for WorldExpo and Mall. The result for our approach show the mean over 5 random trails with standard deviation (\%) for 5 unlabeled images / depth images}
%	\bgroup
%	\def\arraystretch{1.15}% 
	\begin{tabular}{||l|c|c||c|c||}
		\hline
		\multirow{2}{*}{\textbf{Models}} &
		\multicolumn{2}{c||}{\textbf{WorldExpo}} & \multicolumn{2}{c||}{\textbf{WorldExpo} $\rightarrow$ \textbf{Mall}}  \\ \cline{2-5} 
		& \textbf{MAE} & \textbf{RMSE} & \textbf{MAE} & \textbf{RMSE} \\ \hline
		% ResNet: WE
		FCN~\cite{he2016deep}  &23.07& 34.16& 9.03    & 9.6 \\ 
		FCN w/ BN~\cite{he2016deep} &21.65&33.3& 9.63    & 10.32\\ 
		\textbf{Ours (RGB) w/ FCN}  &\textbf{\color{blue}{20.90 $\pm {\tiny 0.1}$}}&\textbf{\color{red}{29.59 $\pm {\tiny 0.07}$}}&  \textbf{\color{red}{4.10 $\pm {\tiny 0.1}$}}   & \textbf{\color{red}{5.10 $\pm {\tiny 0.1}$}}  \\ 
		\textbf{Ours (depth) w/ FCN}  &\textbf{\color{red}{20.22 $\pm {\tiny 0.1}$}}&\textbf{\color{blue}{29.77 $\pm {\tiny 0.1}$}}& \textbf{\color{blue}{6.25 $\pm {\tiny 0.8}$}}     & \textbf{\color{blue}{7.24 $\pm {\tiny 0.7}$}}     \\ \hline
		
		% ResNet SFCN: WE
		SFCN~\cite{wang2019learning}    & 25.47 & 35.91 &  15.17   &  15.53   \\ 
		SFCN w/ BN~\cite{wang2019learning}  & 23.84 & 35.52 & 10.8    &  11.39\\  
		\textbf{Ours (RGB) w/ SFCN} &\textbf{\color{blue}{14.55 $\pm {\tiny 0.1}$}}&\textbf{\color{blue}{22.73$\pm {\tiny 0.1}$}}& \textbf{\color{red}{6.79 $\pm {\tiny 1.3}$}}   & \textbf{\color{red}{7.79 $\pm {\tiny 1.1}$}} \\ 
		\textbf{Ours (depth) w/ SFCN}   &\textbf{\color{red}{13.48 $\pm {\tiny 0.2} $}}&\textbf{\color{red}{22.68$\pm {\tiny 0.3} $}}& \textbf{\color{blue}{8.15$\pm {\tiny 0.2}$}}     & \textbf{\color{blue}{9.08 $\pm {\tiny 0.1}$}}     \\ \hline
	\end{tabular}
	\label{tab:we_other_5shot}
\end{table*}


==> tables/tab_we_pets_fdst.tex <==
\begin{table*}[]
	\label{tab:we_pets_fdst}
	\centering
	\caption{Quantitative results for WorldExpo to PETS and WorldExpo to FDST}
%	\bgroup
%	\def\arraystretch{1.15}% 
	\begin{tabular}{||l|c|c||c|c||}
		\hline
		\multirow{2}{*}{\textbf{Models}} & \multicolumn{2}{c||}{\textbf{WorldExpo} $\rightarrow$ \textbf{PETS}} & \multicolumn{2}{c||}{\textbf{WorldExpo} $\rightarrow$ \textbf{FDST}} \\ \cline{2-5} 
		&  \textbf{MAE} $(\downarrow)$                   & \textbf{MSE} $(\downarrow)$                  & \textbf{MAE} $(\downarrow)$               & \textbf{MSE} $(\downarrow)$               \\ \hline
		CSRNet ~\cite{li2018csrnet}      &  17.99   &  19.80  &       12.74    &  13.09          \\ 
		CSRNet w/ BN~\cite{li2018csrnet}         &  18.63   &  20.49     &   7.30 &  7.81  \\ 
		{\fontfamily{qcr}\selectfont AdaCrowd} + RGB (\textbf{Ours})       &  \textbf{\color{red}{17.43 $\pm {\tiny 0.04} \%$}}   &  \textbf{\color{blue}{19.70 $\pm {\tiny 0.05} $}}       &  \textbf{\color{blue}{7.14 $\pm {\tiny 0.3} $}}   &   \textbf{\color{blue}{7.7 $\pm {\tiny 0.2} $}}    \\ 
		{\fontfamily{qcr}\selectfont AdaCrowd} + Depth (\textbf{Ours})       & \textbf{\color{blue}{17.95 $\pm {\tiny 2.9} \% $}}     & \textbf{\color{red}{19.29 $\pm {\tiny 2.3} \% $}}    & \textbf{\color{red}{6.99 $\pm {\tiny 0.6} \% $}}     & \textbf{\color{red}{7.5 $\pm {\tiny 0.6} \% $}}      \\ \hline
		
		% ResNet: WE
		ResNet101~\cite{he2016deep}        &  20.38   & 22.67  &  7.14   &  7.85  \\ 
		ResNet101 w/ BN~\cite{he2016deep}    &  19.59   &  21.61     &  8.89   &  9.23        \\ 
		{\fontfamily{qcr}\selectfont AdaCrowd} + RGB (\textbf{Ours})    & \textbf{\color{red}{13.74 $\pm {\tiny 0.1} \% $}}     & \textbf{\color{red}{16.15 $\pm {\tiny 0.09} \% $}}     &  \textbf{\color{red}{6.13 $\pm {\tiny 0.4} $}}   & \textbf{\color{red}{6.69 $\pm {\tiny 0.3} $}}         \\ 
		{\fontfamily{qcr}\selectfont AdaCrowd} + Depth (\textbf{Ours})    & \textbf{\color{blue}{19.56 $\pm {\tiny 3.1} \% $}}     & \textbf{\color{blue}{21.52 $\pm {\tiny 2.5} \% $}}      & \textbf{\color{blue}{7.07 $\pm {\tiny 0.3} \% $}}     & \textbf{\color{blue}{7.71$\pm {\tiny 0.3} \% $}}     \\ \hline
		
		% ResNet SFCN: WE
		ResNet101 SFCN~\cite{wang2019learning}      &  19.62   &  21.55     &  8.72 & 8.94   \\ 
		ResNet101 SFCN w/ BN~\cite{wang2019learning}   &  19.94   &  22.26  &  6.60   &  6.96  \\  
		{\fontfamily{qcr}\selectfont AdaCrowd} + RGB (\textbf{Ours})  & \textbf{\color{blue}{18.41 $\pm {\tiny 0.2} $}}  & \textbf{\color{blue}{20.63 $\pm {\tiny 0.1} $}} &  \textbf{\color{red}{5.76 $\pm {\tiny 0.3} $}}   &  \textbf{\color{red}{6.57 $\pm {\tiny 0.3} $}}  \\ 
		{\fontfamily{qcr}\selectfont AdaCrowd} + Depth (\textbf{Ours})     & \textbf{\color{red}{13.74 $\pm {\tiny 0.1} \% $}}     & \textbf{\color{red}{16.15 $\pm {\tiny 0.09} \% $}}      & \textbf{\color{blue}{5.99 $\pm {\tiny 0.6} \% $}}     & \textbf{\color{blue}{6.61 $\pm {\tiny 0.5} \% $}}      \\ \hline
	\end{tabular}
\end{table*}

